Speaker Embeddings as Individuality Proxy for Voice Stress Detection

Since the mental states of the speaker modulate speech, stress introduced by cognitive or physical loads could be detected in the voice. The existing voice stress detection benchmark has shown that the audio embeddings extracted from the Hybrid BYOL-S self-supervised model perform well. However, the benchmark only evaluates performance separately on each dataset, but does not evaluate performance across the different types of stress and different languages. Moreover, previous studies found strong individual differences in stress susceptibility. This paper presents the design and development of voice stress detection, trained on more than 100 speakers from 9 language groups and five different types of stress. We address individual variabilities in voice stress analysis by adding speaker embeddings to the hybrid BYOL-S features. The proposed method significantly improves voice stress detection performance with an input audio length of only 3-5 seconds.

==> 04_Discussion.tex <==


The effect of a stimulus on an individual's perception can be highly dependent on individuality factors such as their personality traits and current emotional state~\cite{bias_personality_analysis}. For instance, in~\cite{personalized_task_load_prediction}, it is shown that a significant relationship exists between a listener's perceived task load and their personality and frustration intolerance, which were measured for each individual through questionnaires. For instance, an easily frustrated individual will tend to perceive tasks to be more demanding than an individual with a higher tolerance for frustration. Consequently, extracting information about a speaker's individuality factors can enable a more accurate prediction of their perceived cognitive load. We, therefore, hypothesize that extracting speaker identity embeddings can improve the prediction of a speaker's perceived cognitive load. Indeed, these embeddings can act as a proxy to certain individuality factors, information about which is embedded within their speech.
